Hadronic and radiative decays of the tau lepton

This PhD thesis studies some hadronic and radiative decays of the tau lepton using a Chiral Lagrangian including resonance fields. After a theoretical introduction, the decays to the $(\pi \pi \pi)^-$, $(KK\pi)^-$ and $\eta^{(\prime)} \pi^- \pi^0$ hadronic states and $\tau \to (\pi/K)^- \gamma \nu_tau$ are analysed. Some material, which was not included in the corresponding references, is also discussed: The structure functions analysis for the 3 pion modes, the differential decay width as a function of the two-particle invariant masses in the considered three-meson modes and a simplified study of the $\tau\to$\eta^{(\prime)} \pi^- \pi^0 \nu_tau$ processes within a single-angle mixing scheme for the $\eta$ and $\eta^\prime$ mesons.

==> phasespace.tex <==
\chapter*{Appendix A: Phase-space integration in $\tau^-\rightarrow(h_1 h_2 h_3)^- \nu_\tau$}
\label{App_phasespace}
\addcontentsline{toc}{chapter}{Appendix A: Phase-space integration in $\tau^-\rightarrow(h_1 h_2 h_3)^- \nu_\tau$}
\appendix
\pagestyle{appendixa}
\newcounter{A}
\renewcommand{\thesection}{\Alph{A}}
\renewcommand{\theequation}{\Alph{A}.\arabic{equation}}
\setcounter{A}{1}
\setcounter{equation}{0}
